Beyond Voice Identity Conversion: Manipulating Voice Attributes by Adversarial Learning of Structured Disentangled Representations

Voice conversion (VC) consists of digitally altering the voice of an individual to manipulate part of its content, primarily its identity, while maintaining the rest unchanged. Research in neural VC has accomplished considerable breakthroughs with the capacity to falsify a voice identity using a small amount of data with a highly realistic rendering. This paper goes beyond voice identity and presents a neural architecture that allows the manipulation of voice attributes (e.g., gender and age). Leveraging the latest advances on adversarial learning of structured speech representation, a novel structured neural network is proposed in which multiple auto-encoders are used to encode speech as a set of idealistically independent linguistic and extra-linguistic representations, which are learned adversariarly and can be manipulated during VC. Moreover, the proposed architecture is time-synchronized so that the original voice timing is preserved during conversion which allows lip-sync applications. Applied to voice gender conversion on the real-world VCTK dataset, our proposed architecture can learn successfully gender-independent representation and convert the voice gender with a very high efficiency and naturalness.

==> abstract.tex <==
\vspace{-0.25cm}
\begin{abstract}
Non-negative matrix factorization (NMF) is a dictionary learning technique which consists into the decomposition of a signal into non-negative elementary parts. The non-negative matrix deconvolution (NMD) is the convolutive formulation of the NMF, convolutive architectures being extremely effectives in many machine learning tasks.
Recently, supervised variants of the NMF have been successfully introduced for separation, detection,  and classification tasks in which the dictionaries are learned from annotated data. However, this is highly restrictive since its requires time-consuming manual annotations which can be accomplished only from a limited amount of data. This paper establishes a slightly-supervised dictionary learning algorithm, which can be learned from partially annotated and noisy data. The proposed algorithm is inspired from joint factor analysis, in which multiple factors are learned simultaneously with different objectives in order to capture different aspects from the same data. This can typically be used to learn dictionaries from noisy data, for which multiple instances of the same object are available, but assuming specific noise associated with each instance. Moreover, a mini-batch version of the proposed algorithm is described which ensures its scalability to large databases. The proposed algorithm is illustrated on the bird audio detection challenge.
% Historically, NMF has been used used for wide range of applications, including sparse coding and blind source separation and for a wide range of textual, image, audio, and bio signals. 
\vspace{0.3cm}
\end{abstract}

\begin{keywords}
non-negative matrix factorization, joint factor analysis, slightly supervised learning, mini-batch learning.
\vspace{-0.1cm}
\end{keywords}

